Efficient Automatic Tuning for Data-driven Model Predictive Control via Meta-Learning

AutoMPC is a Python package that automates and optimizes data-driven model predictive control. However, it can be computationally expensive and unstable when exploring large search spaces using pure Bayesian Optimization (BO). To address these issues, this paper proposes to employ a meta-learning approach called Portfolio that improves AutoMPC's efficiency and stability by warmstarting BO. Portfolio optimizes initial designs for BO using a diverse set of configurations from previous tasks and stabilizes the tuning process by fixing initial configurations instead of selecting them randomly. Experimental results demonstrate that Portfolio outperforms the pure BO in finding desirable solutions for AutoMPC within limited computational resources on 11 nonlinear control simulation benchmarks and 1 physical underwater soft robot dataset.

==> algorithm/greedy_portfolio.tex <==
% \begin{algorithm}[t]
%  \caption{\label{alg:port} Greedy Portfolio Construction.}
%  \begin{algorithmic}[1]
%    \STATE \textbf{Input:} Set of candidate System ID models $C$, $D_{meta} = \{ D_1, \ldots, D_{|meta|} \}$, maximal portfolio size $p$.  
%    % \STATE Randomly partition $\ds_I \cup \ds_H = \ds$, $\ds_I \cap \ds_H = \varnothing$
%    \STATE \FOR{$i \gets 1$ to $n$} \label{lst:line:train_bootstraps}
%      \STATE bootstrap\_sample $\gets$ resample($\ds_H$)
%      \STATE $\hat{f}_{surr,i}$ $\gets$ \texttt{TRAIN}(bootstrap\_sample, $h_{surr}$)
%    \ENDFOR
%    \STATE history = \{ \} \\
%    \STATE \FOR{$i \gets 1$ to $n$} \label{lst:line:main_loop_extended}
%      \STATE $h$ $\gets$ \texttt{BAYES-OPT}(history)
%      \STATE $\hat{f}_{sysid}$ $\gets$ $\texttt{TRAIN}(\ds_I, h)$
%      \STATE optimizer $\gets$ $\texttt{BUILD-OPTIMIZER}(h)$
%      \STATE $\Jdist$ $\gets$ $\{ \}$
%      \STATE \FOR{$j \gets 1$ to $N$} \label{lst:line:task_loop} 
%        \STATE $\objf$ $\gets$ $\texttt{Transformer}(\task_j, h)$
%        \STATE controller $\gets$ \texttt{BUILD-CONTROLLER}($\hat{f}_{sysid}$, $\objf$, optimizer)
%        \STATE \FOR{$k \gets 1$ to $M$} \label{lst:line:bootstrap_eval_loop}  
%          \STATE trajectory $\gets$ \texttt{SIMULATE}(controller, $\hat{f}_{surr,k}$, $\task_j$)
%          \STATE score $\gets$ \texttt{SCORE}(trajectory, $\task_j$)
%          \STATE $\Jdist \gets \Jdist \cup \{ \textrm{score} \}$
%        \ENDFOR
%      \ENDFOR
%      \STATE history $\gets$ history $\cup$ $\{ (h, \texttt{AGGREGATE}(\Jdist) ) \}$
%      \ENDFOR
%    \STATE \textbf{Return} $h$ with minimum $\texttt{AGGREGATE}(\Jdist)$
   
%  \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[t]
 \caption{\label{alg:port} Greedy Portfolio Building}
 \begin{algorithmic}[1]
   \STATE \textbf{Input:} Candidate $C=\{h_1, \ldots, h_l \}$, Set of meta-datasets $D_{meta}=\{D_1, \ldots, D_{|D_{meta}|} \}$, maximal portfolio size $p$.  

   % \STATE $P = \emptyset$, $C = \emptyset$
   % \STATE
   
   % \STATE \textit{// Construct candidate $C$.}
   % \FOR{$D_d \gets D_1$ to $D_{|D_{meta}|}$}
   %      \STATE $h_d=\{\}$
   %      \FOR{$i \gets 1$ to $3$}
   %      % \STATE Randomly partition $D_{d,train} \bigcup D_{d,test} = D_d$, $D_{d,train} \bigcap D_{d,test} = \emptyset$
   %      % \STATE $h_{d,i} \in \text{argmin}_{h \subseteq \mathcal{H}_S} \widehat{GE}(h,D_d)$
   %      \STATE $(h_{d,i}, \widehat{GE}_i)$
        
   %      \ENDFOR
   % \ENDFOR

   % \STATE
   
   \WHILE{$|P| < p$}
        \STATE $h^+ \in \text{argmin}_{h \in C}  \ \hat{\epsilon}_{S}(P\bigcup \{h\}, D_{meta}) $
        \STATE $P=P \bigcup \{h^+\}$, $C=C \setminus  \{h^+\}$
   \ENDWHILE
   
   \STATE \textbf{Return} Portfolio $P$
   
 \end{algorithmic}
\end{algorithm}

==> table/port_best.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[htbp]
\caption{Results of the \texttt{AutoMPC} with portfolio. \todo{TODO}}
\label{tb:port}
\small
\begin{center}
\resizebox{1.0\linewidth}{!}{
\fontsize{20}{35}\selectfont
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{c|}{} & \multicolumn{4}{c|}{\textbf{RMSE}} &  \\
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{\textbf{BO}} & \multicolumn{2}{c|}{\textbf{Portfolio}} &  \\
\multicolumn{1}{c|}{\multirow{-3}{*}{\textbf{Dataset}}} & \textbf{mean} & \multicolumn{1}{c|}{\textbf{std}} & \textbf{mean} & \multicolumn{1}{c|}{\textbf{std}} & \multirow{-3}{*}{\textbf{Gains (\%)}} \\ \hline
\multicolumn{1}{c|}{HopperSmall} & 0.5987 & \multicolumn{1}{c|}{0.0107} & \textbf{0.5825} & \multicolumn{1}{c|}{0.0059} & \textit{2.7059} \\
\multicolumn{1}{c|}{Walker2dSmall} & 12.9722 & \multicolumn{1}{c|}{0.2790} & \textbf{12.7447} & \multicolumn{1}{c|}{0.1073} & \textit{1.7538} \\
\multicolumn{1}{c|}{InvertedPendulumSmall} & 1.2506 & \multicolumn{1}{c|}{0.0555} & \textbf{1.2182} & \multicolumn{1}{c|}{0.0205} & \textit{2.5908} \\
\multicolumn{1}{c|}{HalfCheetahGravityHalf} & 2.5899 & \multicolumn{1}{c|}{0.0214} & \textbf{2.5499} & \multicolumn{1}{c|}{0.0234} & \textit{1.5445} \\
\multicolumn{1}{c|}{HopperGravityOneAndHalf} & 0.8803 & \multicolumn{1}{c|}{0.0361} & \textbf{0.8402} & \multicolumn{1}{c|}{0.0159} & \textit{4.5553} \\
\multicolumn{1}{c|}{HumanoidGravityHalf} & 5.5249 & \multicolumn{1}{c|}{0.0849} & \textbf{5.4366} & \multicolumn{1}{c|}{0.0589} & \textit{1.5982} \\
\multicolumn{1}{c|}{HalfCheetahSmallLeg} & 2.5504 & \multicolumn{1}{c|}{0.0340} & \textbf{2.5358} & \multicolumn{1}{c|}{0.0077} & \textit{0.5725} \\
\multicolumn{1}{c|}{HopperBigThigh} & 0.8194 & \multicolumn{1}{c|}{0.0233} & \textbf{0.8090} & \multicolumn{1}{c|}{0.0085} & \textit{1.2692} \\
\multicolumn{1}{c|}{HopperSmallTorso} & 0.8656 & \multicolumn{1}{c|}{0.0429} & \textbf{0.8060} & \multicolumn{1}{c|}{0.0066} & \textit{6.8854} \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{329A9D}\textit{\textbf{Out-of-distribution Data}}} \\ \hline
\multicolumn{1}{c|}{Cartpole} & 0.0101 & \multicolumn{1}{c|}{0.0007} & \textbf{0.0088} & \multicolumn{1}{c|}{0.0012} & \textit{12.8713} \\
\multicolumn{1}{c|}{Pendulum} & \textbf{0.3174} & \multicolumn{1}{c|}{0.0000} & 0.3174 & \multicolumn{1}{c|}{0.0000} & \textit{0.0000} \\
\multicolumn{1}{c|}{Underwater Soft Robot} & \textbf{0.1165} & \multicolumn{1}{c|}{0.0000} & \textbf{0.1165} & \multicolumn{1}{c|}{0.0000} & \textit{0.0000} \\ \hline
\end{tabular}}
\end{center}
\end{table}
